Client-CASH: Protecting Master Passwords against Offline Attacks

Offline attacks on passwords are increasingly commonplace and dangerous. An offline adversary is limited only by the amount of computational resources he or she is willing to invest to crack a user's password. The danger is compounded by the existence of authentication servers who fail to adopt proper password storage practices like key-stretching. Password managers can help mitigate these risks by adopting key stretching procedures like hash iteration or memory hard functions to derive site specific passwords from the user's master password on the client-side. While key stretching can reduce the offline adversary's success rate, these procedures also increase computational costs for a legitimate user. Motivated by the observation that most of the password guesses of the offline adversary will be incorrect, we propose a client side cost asymmetric secure hashing scheme (Client-CASH). Client-CASH randomizes the runtime of client-side key stretching procedure in a way that the expected computational cost of our key derivation function is greater when run with an incorrect master password. We make several contributions. First, we show how to introduce randomness into a client-side key stretching algorithms through the use of halting predicates which are selected randomly at the time of account creation. Second, we formalize the problem of finding the optimal running time distribution subject to certain cost constraints for the client and certain security constrains on the halting predicates. Finally, we demonstrate that Client-CASH can reduce the adversary's success rate by up to $21\%$. These results demonstrate the promise of the Client-CASH mechanism.

==> 3P_gains.tex <==
We have that, in general, 
\begin{equation*}
\begin{split}
\hprob{i} & = \frac{O_i}{W}e^{\epsilon u'(i)}\\
W & = O_1 + O_2e^{-\epsilon/2} + O_3e^{-\epsilon}
\end{split}
\end{equation*}
For this analysis, we assume that $\ell_1 = \ell_2 = 3 \Rightarrow (O_1,O_2,O_3) = (3,2,4)$. We now have by \textsection 5.1 that $\padv$ is the smallest real number such that the following hold:\\
\\
If $\pwdratio \le 1$:
\begin{equation*}
\begin{split}
\padv& \ge \pwdratio \left(\frac{3}{5}\hprob{1} + \frac{3}{5}\hprob{2} \right)\\
\padv & \ge \frac{9}{19}\pwdratio\\
\padv & \ge \pwdratio \hprob{1}\\
\end{split}
\end{equation*}
If  $\pwdratio \in \left[1,\frac{19}{9}\right]$: \\
$\padv \ge \hprob{1} + \hprob{2} + \left( \pwdratio\frac{9}{4} - \frac{15}{4} \right)\hprob{3}$\\
$\padv \ge \frac{3}{2}\left( \hprob{1} + \hprob{2} + \left(\pwdratio\frac{3}{2}-\frac{15}{4} \right)\hprob{3}  \right)$\\
$\padv \ge \hprob{1} + \frac{9}{10}\left( \pwdratio - 1 \right) (\hprob{2} + \hprob{3})$\\
\\
If we additionally have $\pwdratio \in \left[ 1,\frac{5}{3} \right]$:\\
$\padv \ge \hprob{1} + \frac{3}{2}\left(  \pwdratio - 1\right)\hprob{2}$\\
\\
Below is a graph of the results. 
\begin{figure}[h!]
\centering
\includegraphics[scale=0.4]{threepred_graphs.png}
\caption{Gain plots for three rounds using the exponential mechanism for various values of $\epsilon$. Values of $e^{-\epsilon}$ range from 0-0.3 (top left), 0.3-0.5 (top right), 0.5-0.8 (bottom left) and 0.8-1.0 (bottom right).  }
\label{fig:threepred}
\end{figure}

\anote{ These graphs have many intersection points, which lead me to believe that this distribution is farther from optimal than we may want - perhaps an exponential distribution isn't quite optimal? Still need to solve the linear program for the three round case and generate graphs. 
}

==> adv_opt.tex <==
For a fixed number of rounds $n$, define $\{\advstrat{i}\}_{i \in \{1,2,...n\}}$ to be a family of strategies of the adversary such that with strategy $\advstrat{j}$ for some fixed $j$, the adversary will maximize the number of passwords that he can hash $j$ times. It is also important to note that the sets the adversary picks for his strategy depends on $\pwdratio$. Formally, we can define $\advstrat{i}$ to satisfy the following conditions. 

\begin{equation*}
\begin{split}
\advstrat{i} & : \mathbb{R}^+ \to F\\
\advstrat{i}\left( \pwdratio \right) & = \mathbf{b} \text{ such that } \forall \mathbf{b'} \in F, b_i \ge b'_i
\end{split}
\end{equation*}
$\advstrat{i}$ is well defined - there can only be one output for a specific value of $\pwdratio$ due to the nature of the constraints that define $F$. The construction of $\advstrat{i}\left( \pwdratio \right)$ is as follows. We wish to maximize $b_i$. However, we have an upper bound on $b_i$, given by $$
b_i \le \frac{\ell_{i-1}-1}{\ell_i} b_{i-1}
$$
since this is the only bound on $b_i$, we make the inequality an equality to maximize $b_i$, so we have $b_{i-1}$ in terms of $b_i$. Repeating the process, we work our way up the chain of inequalities (which we then make equalities) to obtain, in general, for some $j < i$, $$
b_j  = \left( \prod\limits_{t = j}^i \frac{\ell_t}{\ell_{t-1}-1} \right) b_i. 
$$
Lastly, to maximize $b_i$, for $m > i$ we set $b_m$ to be as small as possible. Ideally, we set it to zero unless some of the budget is left over after executing the strategy to its completion. However, this only occurs when $\pwdratio > 1$, and the exact amount left over depends on the value of $\pwdratio$. Thus we obtain a unique strategy vector $\mathbf{b}$ and $\advstrat{i}$ is well defined. \\
\\
Moreover, we claim that strategies given by $\advstrat{i}$ are dominant, optimal strategies for the adversary. \anote{ Need to give more details on why, or put a proof in here somewhere...} \\
\\
Define $f(\mathbf{b}) = \sum\limits_{i=1}^n \hprob{i}b_i \left(  \frac{n}{n-1} \right)^{i-1}$. Then 

\begin{equation*}
\begin{split}
\padv & = \pwdratio\max f(\mathbf{b})\\
& = \pwdratio \max\limits_i f\left( \advstrat{i}\left(  \pwdratio  \right) \right)
\end{split}
\end{equation*}
which gives us at most $n$ values to calculate, a much more efficient way of finding $\padv$ than formulating it as a linear program and solving it. This formulation is also very powerful since it gives us information about $\padv$ even when the $\hprob{j}$'s are not known. 

==> adv_opt_strat.tex <==
Calculating the optimal $\padv$ for fixed $\hprob{j}$'s may be made efficient if we consider \textit{dominant strategies} of the adversary; i.e. $\mathbf{b^*} \in F$ which yield greater values of $\padv$ than other $\mathbf{b} \in F$ independent of the values of $\hprob{j}$'s. For some $S \subseteq F$, let $\advstrat{i}(S) \subseteq S$ denote the collection of members of $S$ such that $b_i$ is maximized. Formally, we define for all $S \subseteq F$,$$
\advstrat{i}(S) := \{\mathbf{b} \in S: \forall \mathbf{b'} \in S, b_i \ge b'_i\}
$$
Then we claim that the collection $F^* := \bigcup\limits_{i=1}^n \advstrat{i}(F)$ is the collection of dominant strategies of the adversary. 

\newcommand{\thmadvstrat}{
Let $F^* := \bigcup\limits_{i=1}^n \advstrat{i}(F)$. Then 

\begin{equation*}
\begin{split}
\padv &= \pwdratio \max\limits_{\mathbf{b} \in F}\left\{
\hprob{1}b_1 + \sum\limits_{i=2}^n \hprob{i}b_i \prod\limits_{j=1}^{i-1} \left(\frac{\ell_j}{\ell_j - 1} \right)
\right\}\\
& = \pwdratio \max\limits_{\mathbf{b} \in F^*}\left\{
\hprob{1}b_1 + \sum\limits_{i=2}^n \hprob{i}b_i \prod\limits_{j=1}^{i-1} \left(\frac{\ell_j}{\ell_j - 1} \right)
\right\}
\end{split}
\end{equation*}
}

\begin{theorem}
\label{thm:advstrat}
\thmadvstrat
\end{theorem}

The proof can be found in the appendix. \\
\\
\anote{Will add more intuitive explanations of formulation and the theorem in this section.}\\

==> adv_strat2.tex <==
We can find potentially optimal strategies for the adversary independent of the probability distribution of the outcome selection. When $n=2$ and $\ell_1 = 2$,  $$
\padv = \pwdratio\max\limits_{\mathbf{b} \in F} \left\{  \hprob{1}b_1 + 2\hprob{2}b_2  \right\}
$$
When $\hprob{1}$ and $\hprob{2}$ are fixed, we can formulate the above as the following linear program. \\
\\
\textbf{maximize } $\pwdratio \left(  \hprob{1}b_1 + 2\hprob{2}b_2 \right)$\\
\textbf{subject to }  \\
(1) $b_1,b_2 \in \left[ 0, \min\left\{ 1,\invpwdratio \right\}  \right]$\\
(2) $b_1 + b_2 = 1$\\
(3) $b_2 \le \frac{1}{2}b_1$\\
\\
Rewriting the above constraints using $b_2 = 1-b_2$, we have \\
\\
\textbf{maximize } $\pwdratio \left( (\hprob{1} - 2\hprob{2})b_1 + 2\hprob{2} \right)$\\
\textbf{subject to }\\
(1) $b_1 \in \left[ 0, \min\left\{ 1,\invpwdratio \right\}  \right]$\\
(2) $b_2 \ge 1 - \invpwdratio$\\
(3) $b_1 \ge \frac{2}{3}$\\
\\
However, we note that constraint (2) gives us no extra information as (3) is a tighter bound on $b_1$. Thus, we have that $b_1 \in \left[ \frac{2}{3}, \min\left\{ 1,\invpwdratio \right\}  \right]$. Since our objective function is linear, it is clear that the optimal $b_1$ occurs at the endpoints of the interval. \\
\\
$b_1 = \frac{2}{3} \Rightarrow \padv \ge \frac{2}{3}\pwdratio$\\
\\
If $\pwdratio < 1$, then we also have $b_1 = 1 \Rightarrow \padv \ge \pwdratio \hprob{1}$\\
Else if $1 \le \pwdratio \le \frac{3}{2}$ we have $\padv \ge \hprob{1} - 2\hprob{2} + \pwdratio 2\hprob{2}$\\
\\
Thus the constraint stating that $$
\padv = \pwdratio\max\limits_{\mathbf{b} \in F} \left\{  \prob{1}b_1 + 2\prob{2}b_2  \right\}
$$
can be replaced by the following two constraints. 
\begin{itemize}
\item $\padv \ge \frac{2}{3}\pwdratio$
\item $\padv \ge \begin{cases}
\prob{1}\pwdratio & \text{ if } \pwdratio \le 1\\
\prob{1} + 2\left(  \pwdratio - 1 \right) \prob{2} & \text{ otherwise }
\end{cases}$
\end{itemize}





==> adv_strat3.tex <==
Finding the optimal strategies for the adversary reduces to calculating $\advstrat{1},\advstrat{2}$ and $\advstrat{3}$ for different values of $\pwdratio$. When $\pwdratio \le 1$, it is easy to see that

\begin{equation*}
\begin{split}
\advstrat{1}\left( \pwdratio \right) & = (1,0,0)\\
\advstrat{2}\left( \pwdratio \right) & = \left(  \frac{3}{5},\frac{2}{5},0  \right)\\
\advstrat{3}\left( \pwdratio \right) & = \left(  \frac{9}{19},\frac{6}{19},\frac{4}{19}   \right)
\end{split}
\end{equation*}
Now suppose that $\pwdratio \ge 1$. Then since $\pwdratio \le \frac{19}{9}$, we still have that $\advstrat{3}\left( \pwdratio  \right) = \left( \frac{9}{19},\frac{6}{19},\frac{4}{19}  \right)$. To find $\advstrat{2}$, we let $b_2 = \frac{2}{3}b_1$ and $b_1 = \min\left\{\invpwdratio,\frac{3}{5}\right\}$ since $\frac{3}{5}$ gives an optimal strategy when $\mathbf{b}$ is less constrained. Thus $$
\advstrat{2}\left(  \pwdratio \right) = 
\begin{cases}
\left(  \frac{3}{5},\frac{2}{5},0  \right) & \text{ if } \pwdratio \in \left[1,\frac{5}{3}\right]\\
\left( \invpwdratio,\frac{2}{3}\invpwdratio,1-\frac{5}{3}\invpwdratio  \right) & \text{ if } \pwdratio \in \left[  \frac{5}{3},\frac{19}{9} \right]
\end{cases}
$$
Lastly, to find $\advstrat{1}\left(  \pwdratio\right)$ we set $b_1 = \invpwdratio$ so that $b_2 + b_3 = 1- \invpwdratio$. There are two options - either a $\advstrat{2}$-like strategy can be implemented, setting $b_3 = 0$, or a $\advstrat{3}$-like strategy is implemented, maximizing $b_3$ given that $b_1 = \invpwdratio$. In the first case, we obtain $\advstrat{1} = \left( \invpwdratio,1-\invpwdratio,0  \right)$ which is only feasible when $\pwdratio \in \left[ 1,\frac{5}{3} \right]$. The other case gives us $\advstrat{1} = \left(  \invpwdratio, \frac{3}{5}\left( 1 - \invpwdratio \right),\frac{2}{5}\left(  1 - \invpwdratio  \right)  \right)$ which is always feasible for $\pwdratio \in \left[1,\frac{19}{9}\right]$. \\
\\
Translating these strategies into constraints for $\padv$, we obtain the following. When $\pwdratio \le 1$, 
\begin{equation*}
\begin{split}
(1) \padv & \ge \hprob{1}\pwdratio\\
(2) \padv & \ge \frac{3}{5}(\hprob{1} + \hprob{2})\pwdratio\\
(3) \padv & \ge \frac{9}{19}\pwdratio
\end{split}
\end{equation*}
When $\pwdratio \in \left[1,\frac{5}{3}\right]$, 

\begin{equation*}
\begin{split}
(4) \padv & \ge \hprob{1} + \frac{3}{2}\hprob{2}\left( \pwdratio - 1  \right)\\
(5) \padv & \ge \hprob{1} + \frac{9}{10}(\hprob{2} + \hprob{3})\left( \pwdratio-1  \right)\\
(6) \padv & \ge \frac{3}{5}(\hprob{1} + \hprob{2})\pwdratio\\
(7) \padv & \ge \frac{9}{19}\pwdratio
\end{split}
\end{equation*}
When $\pwdratio \in \left[ \frac{5}{3},\frac{19}{9} \right]$,

\begin{equation*}
\begin{split}
(8) \padv & \ge \hprob{1} + \frac{9}{10}(\hprob{2} + \hprob{3})\left( \pwdratio-1  \right)\\
(9) \padv & \ge \hprob{1} + \hprob{2} + \frac{9}{4}\hprob{3}\left(\pwdratio - \frac{5}{3} \right)\\
(10) \padv & \ge \frac{9}{19}\pwdratio
\end{split}
\end{equation*}
We can directly see from these constraints that $\padv$ increases with $B^{(k)}$. It is clear that (4) places a higher bound than (1) as $\pwdratio - 1 > 0$ and constraints (6) and (7) are the same as (2) and (3). In addition, $$
(4) \le \hprob{1} + \frac{3}{2}\hprob{2}\left(\frac{5}{3} - 1\right) \le \hprob{1} + \hprob{2} \le (8)
$$
and $$
(6) \le \hprob{1} + \hprob{2} \le (9).
$$
Since the other constraints are shared in the case where $\pwdratio \in \left[1,\frac{5}{3}\right]$. Thus, as the value of $\pwdratio$ transitions from $\left[1,\frac{5}{3}\right]$ to $\left[\frac{5}{3},\frac{19}{9}\right]$, the value of $\padv$ increases with $\pwdratio$. Thus, as we expect, for a fixed number of rounds $k$, the adversary's probability of success increases monotonically with the budget $B$. 





==> exp_gains.tex <==
For a fixed value of $\epsilon$, we have the following. 
\begin{equation*}
\begin{split}
W & = 1 + e^{-\epsilon}\\
\prob{1} & = \frac{1}{W}\\
\prob{2} & = \frac{e^{-\epsilon}}{W}\\
\alpha & = \prob{1} + 2\prob{2}\\
\end{split}
\end{equation*}
Since $\alpha$ is fixed for a fixed $\epsilon$ (and therefore $k$ is fixed), the problem of finding the maximum gain $G$ reduces to finding the minimum $\padv$ - with this value, we can find the optimal gain for the given parameters. We can thus phrase the optimization problem as follows. \\
\\
\textbf{Input Parameters: } $B,C_{srv},\pwdspace,\epsilon,\outputspace$\\
\textbf{Variables: } $\padv$\\
\textbf{minimize } $\padv$\\
\textbf{subject to }\\
(1) $\padv \ge \frac{2}{3}\pwdratio$\\
(2) $\padv \ge \begin{cases}
\prob{1}\pwdratio & \text{ if } \pwdratio \le 1\\
\prob{1} + 2\left(  \pwdratio - 1 \right)\prob{2} & \text{ otherwise }
\end{cases}$\\
\\
which is a trivial optimization to solve for a given value of $\epsilon$. 

\paragraph{Analysis of results. } Figure 1 has the gains given by the exponential mechanism as a function of $\pwdratio$, showing how the gain varies relative to the adversary's budget size. For $\epsilon \in [0,0.5]$, the gain is increasing in $\epsilon$ (bottom graph). This makes sense - when $\epsilon$ is small, increasing its value loosens constraints and the resulting solution must be at least as good as the first. However, after $\epsilon$ reaches a certain value, this increasing gain behavior does not occur anymore (top graph). For $\epsilon \ge 0.5$, some values of $\epsilon$ are more optimal than others in different cases. However, we can see that these curves in general attain smaller and smaller gains, to the point where for $\epsilon = 2.303$, the gains are strictly smaller than all the previous $\epsilon$. This implies that there is some "optimal" range for $\epsilon$ where the maximum gains are achieved. Although this seems strange as we seemingly loosen our constraints when we increase $\epsilon$, this behavior is caused by the dependence of the probability distribution on $\epsilon$ - higher values of $\epsilon$ correspond to a wider gap between the values of $\prob{1}$ and $\prob{2}$, whereas higher $\epsilon$ in the optimization problem simply mean that the gap \textit{may} be wider, but it is not necessarily true. It is therefore likely that in the optimal solution, there is some stationary probability distribution such that for some $\epsilon^* > 0$, choosing any $\epsilon \ge \epsilon^*$ will not change the optimal probability distribution or the gains. 



==> exp_gains3.tex <==
For a fixed value of $\epsilon$, we have the following. 
\begin{equation*}
\begin{split}
W & = 3 + 2e^{-\epsilon/2} +  4e^{-\epsilon}\\
\prob{1} & = \frac{1}{W}\\
\prob{2} & = \frac{e^{-\epsilon/2}}{W}\\
\prob{3} & = \frac{e^{-\epsilon}}{W}\\
\alpha & = 3\prob{1} + 4\prob{2} + 12\prob{3}\\
\end{split}
\end{equation*}
Since $\alpha$ is fixed for a given $\epsilon$ (and therefore $k$ is fixed), the problem reduces to finding the minimum $\padv$ as it did in the two round case - this can be easily found using the optimal strategy bounds calculated in \textsection 5.1. 

\begin{figure}[h!]
\centering
\includegraphics[scale=0.2]{threepred_exp.jpg}
\caption{Gains for the exponential mechanism for different values of $\epsilon$ with a three-round mechanism. 
}
\label{fig:threepred_exp}
\end{figure}

\paragraph{Analysis of results. } Figure 4 shows the gains ($P_{det} - \padv$) given by the exponential mechanism as a function of $\pwdratio$. As in the two round exponential gains, the gains for the three round gains are strictly increasing roughly when $\epsilon \le 0.693$ and there are crossings in the graphs when $\epsilon$ exceeds this value. As before, increasing the value of $\epsilon$ only increases the gains until a point - in Figure 4, the maximum gain occurs when $\epsilon = 1.609$, and there are diminished gains when $\epsilon = 2.303$. As before, it is likely that there exists some $\epsilon^*$ such that for all $\epsilon \ge \epsilon^*$, the gains are no longer increasing. 

==> gains_old.tex <==
We have that 
\begin{equation*}
\begin{split}
\hprob{i} &= \frac{O_i}{W}e^{\epsilon u'(i)}\\
W & = O_1 + O_2e^{-\epsilon/2} + O_3e^{-\epsilon}\\
\end{split}
\end{equation*}
From \textsection 5.1 we have that $\padv$ is the smallest real number such that the following hold, given that we consider the case where $\ell_1 = \ell_2 = 3 \Rightarrow (O_1,O_2,O_3) = (3,2,4)$ with $|\outputspace| = 9$. We thus have
\begin{equation*}
\begin{split}
W & = 3 + 2e^{-\epsilon/2} + 4e^{-\epsilon}\\
\padv \ge & \pwdratio \left( \frac{3}{5}\hprob{1} + \frac{3}{5}\hprob{2} \right)\\
& = \pwdratio \frac{1}{W}\frac{3}{5} \left( O_1 + O_2 e^{-\epsilon/2} \right)\\
& = \pwdratio \frac{1}{W}\frac{3}{5} (3 + 2e^{-\epsilon/2})\\
\padv \ge & \pwdratio \hprob{1} \\
& = \pwdratio \frac{O_1}{W} = \pwdratio \frac{3}{W}\\
\padv \ge & \pwdratio \frac{9}{19}
\end{split}
\end{equation*}
It is not hard to see that the first constraint is larger than the second when $\epsilon \le 2\ln \left( \frac{3O_2}{2O_1} \right) = 0$ - thus the second constraint is always larger than the first. In addition,  we have that the second constraint is larger than the third when $\epsilon  \ge 0.723$ - otherwise the third constraint is the largest. \\
\\
Recall that $$
G = 
\begin{cases}
\frac{1}{\alpha}\pwdratio - \padv & \text{ if } \alpha \ge \pwdratio \\
1 - \padv & \text{ otherwise} 
\end{cases}
$$
where 
\begin{equation*}
\begin{split}
\alpha & = \hprob{1} + 2\hprob{2} + 3\hprob{3}\\
& = \frac{1}{W}(3 + 4e^{-\epsilon/2} + 12e^{-\epsilon})\\
& = \frac{3 + 4e^{-\epsilon/2} + 12e^{-\epsilon}}{3 + 2e^{-\epsilon/2} + 4e^{-\epsilon}}
\end{split}
\end{equation*}
\textbf{Case 1: $\epsilon \le 0.723$. }\\
\\
Since $\padv = \pwdratio \frac{9}{19}$, 
$$
G = 
\begin{cases}
\pwdratio \left( \frac{3 + 2e^{-\epsilon/2} + 4e^{-\epsilon}}{3 + 4e^{-\epsilon/2} + 12e^{-\epsilon}} - \frac{9}{19}  \right) & \text{ if } \pwdratio \le \alpha\\
1 - \pwdratio \frac{9}{19} & \text{ otherwise}
\end{cases}
$$
\textbf{Case 2: $\epsilon \ge 0.723$. }\\
\\
Since $\padv = \pwdratio \frac{3}{W}$, 
$$
G = 
\begin{cases}
\pwdratio \left(  \frac{3+2e^{-\epsilon/2} + 4e^{-\epsilon}}{3 + 4e^{-\epsilon/2} + 12e^{-\epsilon}} - \frac{3}{W}  \right) & \text{ if } \pwdratio \le \alpha\\
1 - \pwdratio \frac{3}{W} & \text{ otherwise}
\end{cases}
$$

==> linopt3.tex <==
As before, define $\prob{i}$ to be the probability that an arbitrary and fixed $o \in \outputspace_{i,pwd}$ is selected. Then, for $\ell_j = n$ for all $j$, we have that $(O_1,O_2,O_3) = (3,2,4)$. Thus, 

\begin{equation*}
\begin{split}
\hprob{1} & = 3\prob{1}\\
\hprob{2} & = 2\prob{2}\\
\hprob{3} & = 4\prob{3}
\end{split}
\end{equation*}
We can thus phrase our linear program as follows. \\
\\
\textbf{Input Parameters: } $C_{srv}, \epsilon, \outputspace$\\
\textbf{Variables: } $\prob{1},\prob{2},\prob{3}$\\
\textbf{minmize } $\alpha = \hprob{1} + 2\hprob{2} + 3\hprob{3} = 3\prob{1} + 4\prob{2} + 12\prob{3}$\\
\textbf{subject to}\\
(1) $\prob{i} \in [0,1]$\\
(2) $\sum\limits_{i=1}^3 \hprob{i} = 1 \Rightarrow 3\prob{1} + 2\prob{2} + 4\prob{3} = 1$\\
(3) $e^{-\epsilon}\prob{2} \le \prob{1} \le e^{\epsilon}\prob{2}$\\
(4) $e^{-\epsilon}\prob{3} \le \prob{1} \le e^{\epsilon} \prob{3}$\\
(5) $e^{-\epsilon}\prob{3} \le \prob{2} \le e^{\epsilon} \prob{3}$\\
(6) $\frac{3}{5}\hprob{1} + \frac{3}{5}\hprob{2} = \frac{9}{5}\prob{1} + \frac{6}{5}\prob{2} \le \frac{9}{19}$\\
(7) $\hprob{1} = 3\prob{1} \le \frac{9}{19} \Rightarrow \prob{1} \le \frac{3}{19}$

==> linprogopt.tex <==
After finding the optimal strategies of the adversary, we can directly phrase our optimization problem as a normal linear program, formulated below. \\
\\
\textbf{Input Parameters: } $C_{srv},\epsilon,\outputspace,B, \pwdspace$\\
\textbf{Variables: } $\prob{1},\prob{2},\alpha$\\
\textbf{maximize } $G$\\
\textbf{subject to }\\
(1) $\prob{1}, \prob{2} \in [0,1]$\\
(2) $\prob{1} + \prob{2} = 1$\\
(3) $e^{-\epsilon}\prob{2} \le \prob{1} \le e^{\epsilon}\prob{2}$\\
(4) $\prob{1} + 2\prob{2} \le \alpha$\\
(5) $\padv \ge \frac{2}{3}\pwdratio$\\
(6) $\begin{cases}
\prob{1}\pwdratio & \text{ if } \pwdratio \le 1\\
\prob{1} + 2\left(  \pwdratio - 1 \right)\prob{2} & \text{ otherwise }\\
\end{cases}$\\
\\
The results of this linear program give the optimal gains for each set of parameters. 

\begin{figure}[h!]
\centering
\includegraphics[scale=0.3]{twopred_opt.jpg}
\caption{Gains for the optimal probability distributions for a wide range of values of $\epsilon$. \anote{I need to fix this graph - the first and immediate change is that the x-axis should be labeled $\pwdratio$. The second thing change is that, since the x-axis is a function of $k$, if we allow $\frac{B}{|\pwdspace|}$ to vary as well, it is not clear what we are seeing. However, if we fix $\frac{B}{|\pwdspace|}$ and allow $k$ to vary as it is, then this graph shows the gain as a function of $k$, not the budget $B$, which shows important results in itself. Specifically, we can find the optimal $k$ for each $\epsilon$.}  }
\label{fig:twopred_opt}
\end{figure}

\paragraph{Analysis of results. } When solving for the gain from the linear program, we do expect that the gain increases as a function of $\epsilon$ and there are thus no crossings as we had in the case with the exponential mechanism. We also cannot have negative gains; we have control over $k$, so we can make the system as close as we want to deterministic and have the gain be 0. Our results clearly satisfy these properties (see Figure 2). In addition, we do see a stationary gain distribution emerge when $\epsilon \ge 0.5$. As with the exponential mechanism, it seems likely that there exists some $\epsilon^*$ such that taking $\epsilon \ge \epsilon^*$ will not change the optimal gains of the system.

\begin{figure}[h!]
\centering
\includegraphics[scale=0.3]{twopred_cmp.jpg}
\caption{Comparison of gains from the exponential and optimal mechanisms. When $\epsilon = 0.511$ (bottom left) and when $\epsilon = 0.223$ (bottom right) the optimal solution's gains with the exponential mechanism's gains. }
\label{fig:twopred_cmp}
\end{figure}

\paragraph{Comparison with the Exponential Mechanism. } We expect that the gains from the optimal distributions is at least as big as the gains from the exponential distribution, and our results satisfy this property (see Figure 3). As $\epsilon$ approaches 0.5, we see that the optimal gains completely match the exponential mechanism gains; however as $\epsilon$ increases beyond this point, the differences in gain become more and more pronounced. However, the exponential mechanism is still optimal for certain values of $\pwdratio$. However, one strength of the exponential mechanism gain distribution is that it uses a fixed value of $k$, and is thus independent of $\frac{B}{|\pwdspace|}$, whereas the optimal results are generating using potentially different values of $k$. Thus, the exponential mechanism could be valuable when we are uncertain of $B$. 










==> linprogopt3.tex <==
As before, we can generate optimal solutions via a normal linear program, formulated below. \\
\\
\textbf{Input Parameters: } $C_{srv}, \epsilon, \outputspace,B,\pwdspace$\\
\textbf{Variables: } $\prob{1}, \prob{2}, \prob{3}, k$\\
\textbf{maximize } $G$\\
\textbf{subject to }\\
(1) $\prob{1},\prob{2},\prob{3} \in [0,1]$\\
(2) $3\prob{1} + 2\prob{2} + 4\prob{3} = 1$\\
(3) $e^{-\epsilon}\prob{j} \le \prob{i} \le e^{\epsilon}\prob{j}$ for $i,j \in \{1,2,3\}$\\
(4) $3\prob{1} + 4\prob{2} + 12\prob{3} \le \alpha$\\
(5a)* If $\pwdratio \le 1$\\
\begin{itemize}
\item $\padv \ge 3\prob{1}\pwdratio$
\item $\left(  \frac{9}{5}\prob{1} + \frac{6}{5}\prob{2}  \right)\pwdratio$
\item $\padv \ge \frac{9}{19}\pwdratio$
\end{itemize}
(5b)* If $\pwdratio \in \left[1,\frac{5}{3}\right]$
\begin{itemize}
\item $\padv \ge 3\prob{1} + 3\prob{2}\left(\pwdratio - 1\right)$
\item $\padv \ge 3\prob{1} + \frac{9}{5}(\prob{2}+2\prob{3})\left( \pwdratio - 1\right)$
\item $\padv \ge \frac{3}{5}(3\prob{1} + 2\prob{2})\pwdratio$
\item $\padv \ge \frac{9}{19}\pwdratio$
\end{itemize}
(5c)* If $\pwdratio \ge \frac{5}{3}$
\begin{itemize}
\item $\padv \ge 3\prob{1} + \frac{9}{5}(\prob{2}+2\prob{3})\left( \pwdratio - 1\right)$
\item $\padv \ge 3\prob{1} + 2\prob{2} + 9\prob{3}\left( \pwdratio - \frac{5}{3}\right)$
\item $\padv \ge \frac{9}{19}\pwdratio$
\end{itemize}

\begin{figure}[h!]
\centering
\includegraphics[scale=0.3]{threepred_opt.jpg}
\caption{Gains for the optimal probability distributions for a wide range of values of $\epsilon$.  }
\label{fig:threepred_opt}
\end{figure}

\paragraph{Analysis of Optimal Results. } As we expect for an optimal solution, the curves in Figure 5 are increasing in $\epsilon$. In addition, we do see a stationary distribution occur as $\epsilon$ increases, with a dome-like top similar to the optimal solutions in the two round system. We additionally have a spike in the gains towards the end of the dome area, corresponding the maximum-gain area of the graph. In addition, we see that the maximum gains are greater than 0.2, a clear increase from two-round mechanisms. 

\begin{figure}[h!]
\centering
\includegraphics[scale=0.3]{threepred_cmp.jpg}
\caption{Comparison between exponential mechanism gains (orange) and optimal mechanism gains (blue) for various values of $\epsilon$. For the cases $\epsilon = 0.511$ (bottom left) and $\epsilon = 0.223$ (bottom right) the optimal and exponential solutions are identical. Otherwise (top left and top right) the exponential mechanism is only optimal for certain ranges of $\pwdratio$.  }
\label{fig:threepred_cmp}
\end{figure}

\paragraph{Comparison with the exponential mechanism. } We expect that the results from the optimal distributions are at least as large as the gains from the exponential mechanism, which is clearly the case (see Figure 6). As in the two-round case, we see that the optimal and exponential distributions begin to diverge as $\epsilon$ becomes larger than 0.5. The exponential mechanism, as before, would be advantageous to use when the value of $\frac{B}{|\pwdspace|}$ is unknown, as the value of $k$ is fixed. It does seem, however, that none of the three-round exponential mechanism gains attain values in the sharp peak between $\pwdratio = 1.5$ and $\pwdratio = 2$, indicating that the exponential mechanism never reaches the most optimal gains. 

\begin{figure}[h!]
\centering
\includegraphics[scale=0.3]{three-twopred_cmp.jpg}
\caption{Comparison between optimal two-round gains (blue) and optimal three-round gains (orange) for various values of $\epsilon$. For $\epsilon = 1.609$ (top left), the three-round gains are always greater than that of the two-round gains, and this is usually the case when $\epsilon = 0.916$ (top right) as well. However, for $\epsilon - 0.511$ (bottom left) and $\epsilon = 0.223$ (bottom right), the two-round optimal gains are greater than the three-round optimal gains until $\pwdratio$ is roughly 1.5. In these cases, the thee-round gains still reach a higher maximum than the two-round gains.}
\label{fig:three-twopred_cmp}
\end{figure}

\paragraph{Comparison with two-round gains. } One of the main differences between the two-round and three-round gains are that in all cases, when $\pwdratio \ge 1.5$ the two-round gains are 0 (as $\padv = 1$), but only when $\pwdratio \ge \frac{19}{9}$ in the three-round case $\padv = 1$ for 0 gains. Thus we allow $\pwdratio$ to take values in a greater range for a greater number of rounds, which is useful if we expect significant variations in the adversary's budget size. In addition, the maximum gains for the three-round systems seem to be always greater than the maximum gains for a two-round system, even though in some cases we have that the two-round gains are greater than the three-round gains for some ranges of $\pwdratio$. The third main difference between the two mechanisms is the value of $k$ - the number of iterations necessary in the three-round case is less than that of the two-round case by a factor of at least $\frac{6}{5}$. \anote{Will put in data for this soon!} This makes sense - we now have the option to use either $k,2k$, or $3k$ hash iterations, so to achieve a comparable level of security we can use a smaller value of $k$. 


